Guide3D: A Bi-planar X-ray Dataset for 3D Shape Reconstruction

Endovascular surgical tool reconstruction represents an important factor in advancing endovascular tool navigation, which is an important step in endovascular surgery. However, the lack of publicly available datasets significantly restricts the development and validation of novel machine learning approaches. Moreover, due to the need for specialized equipment such as biplanar scanners, most of the previous research employs monoplanar fluoroscopic technologies, hence only capturing the data from a single view and significantly limiting the reconstruction accuracy. To bridge this gap, we introduce Guide3D, a bi-planar X-ray dataset for 3D reconstruction. The dataset represents a collection of high resolution bi-planar, manually annotated fluoroscopic videos, captured in real-world settings. Validating our dataset within a simulated environment reflective of clinical settings confirms its applicability for real-world applications. Furthermore, we propose a new benchmark for guidewrite shape prediction, serving as a strong baseline for future work. Guide3D not only addresses an essential need by offering a platform for advancing segmentation and 3D reconstruction techniques but also aids the development of more accurate and efficient endovascular surgery interventions. Our project is available at https://airvlab.github.io/guide3d/.

==> class/localmacros.tex <==
% Macros

\newcommand{\tudor}[1]{\textcolor{blue}{#1}}
\newcommand{\anh}[1]{\textcolor{red}{#1}}
\newcommand{\minh}[1]{\textcolor{magenta}{#1}}
\newenvironment{blue}{\color{blue}}{}
% \def\etal{\emph{et al.}}
\def\ie{\textit{i.e.}}
\def\eg{\textit{e.g.}}
% \newcommand*{\thead}[1]{%
    % \multicolumn{1}{c}{\bfseries\begin{tabular}{@{}c@{}}#1\end{tabular}}}

==> class/packages_setup.tex <==
% to avoid loading the natbib package, add option nonatbib:


% \usepackage{xcolor}
% % \usepackage[utf8]{inputenc} % allow utf-8 input
% % \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% % \usepackage[bookmarks=false]{hyperref}       % hyperlinks
% % \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% % \usepackage{amsfonts}       % blackboard math symbols
% % \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% % \usepackage{microtype}      % microtypography
% % \usepackage{amsthm}
% \usepackage{siunitx}        % for showing units 
% \usepackage{makecell}       % to make the header of the table without much effort
% \usepackage{multirow}       % for multirow

% \usepackage[export]{adjustbox}
% \usepackage{layouts}
% \usepackage{graphicx}
% \usepackage{lipsum}
% \graphicspath{{./}{figures}}

% % \renewcommand\theadfont{\bfseries}

% % \DeclareMathOperator\erf{erf}
% % \newtheorem{proposition}{Proposition}
% % \newtheorem{corollary}{Corollary}[proposition]
% % \theoremstyle{remark}
% % \newtheorem{remark}{Remark}[proposition]
% % \usepackage{floatrow}
% % \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% % \graphicspath{{./}{figures}}

% % \usepackage{subfigure}
% % \usepackage{caption}
% \usepackage{subcaption}

% % \usepackage{amsmath, amssymb}
% \usepackage{csquotes}
% \usepackage{pifont}


\newcommand{\xmark}{\ding{55}}
\newcommand{\cmark}{\ding{51}}


==> figures/architecture.tex <==
 \begin{minipage}[t][][b]{.5\textwidth}
    \adjustimage{left, width=.1\textwidth}{assets/architecture.drawio.png}
    \captionof{figure}{Episode lengths of when utilizing different input modalities.}
    \label{fig:network-architecture}
\end{minipage}

==> figures/spherical.tex <==
 \begin{minipage}[t][][b]{.5\textwidth}
    \adjustimage{left, width=.1\textwidth}{assets/spherical.drawio.png}
    \captionof{figure}{Episode lengths of when utilizing different input modalities.}
    \label{fig:spherical-coordinates}
\end{minipage}
